End-to-end Ensemble-based Feature Selection for Paralinguistics Tasks

The events of recent years have highlighted the importance of telemedicine solutions which could potentially allow remote treatment and diagnosis. Relatedly, Computational Paralinguistics, a unique subfield of Speech Processing, aims to extract information about the speaker and form an important part of telemedicine applications. In this work, we focus on two paralinguistic problems: mask detection and breathing state prediction. Solutions developed for these tasks could be invaluable and have the potential to help monitor and limit the spread of a virus like COVID-19. The current state-of-the-art methods proposed for these tasks are ensembles based on deep neural networks like ResNets in conjunction with feature engineering. Although these ensembles can achieve high accuracy, they also have a large footprint and require substantial computational power reducing portability to devices with limited resources. These drawbacks also mean that the previously proposed solutions are infeasible to be used in a telemedicine system due to their size and speed. On the other hand, employing lighter feature-engineered systems can be laborious and add further complexity making them difficult to create a deployable system quickly. This work proposes an ensemble-based automatic feature selection method to enable the development of fast and memory-efficient systems. In particular, we propose an output-gradient-based method to discover essential features using large, well-performing ensembles before training a smaller one. In our experiments, we observed considerable (25-32%) reductions in inference times using neural network ensembles based on output-gradient-based features. Our method offers a simple way to increase the speed of the system and enable real-time usage while maintaining competitive results with larger-footprint ensemble using all spectral features.

==> related.tex <==
%auto-ignore
%survey of other papers
In this section, we give a brief survey of other solutions for this competition.

==> system_block_diagram.tex <==
%auto-ignore
\begin{tikzpicture}[
    % GLOBAL CFG
    font=\sf \scriptsize,
    >=LaTeX,
    % Styles
    cell/.style={% For the main box
        rectangle, 
        rounded corners=5mm, 
        draw,
        very thick,
        },
    operator/.style={%For operators like +  and  x
        circle,
        draw,
        inner sep=-0.5pt,
        minimum height =.2cm,
        },
    function/.style={%For functions
        ellipse,
        draw,
        inner sep=1pt
        },
    ct/.style={% For external inputs and outputs
        circle,
        draw,
        line width = .75pt,
        minimum width=1cm,
        inner sep=0pt,
        },
    mt/.style={% For external inputs and outputs
        rectangle,
        draw,
        line width = .75pt,
        minimum width=0.5cm,
        inner sep=0pt,
        align=center,
        },
    gt/.style={% For internal inputs
        rectangle,
        draw,
        minimum width=4mm,
        minimum height=3mm,
        inner sep=1pt
        },
    mylabel/.style={% something new that I have learned
        font=\scriptsize\sffamily
        },
    ArrowC1/.style={% Arrows with rounded corners
        rounded corners=.25cm,
        thick,
        },
    ArrowC2/.style={% Arrows with big rounded corners
        rounded corners=.5cm,
        thick,
        },
    ]
    

\node[mt, label=Audio input] (Audio) at (0.5,0)
    {\includegraphics[width=.2\textwidth]{imgs/raw_wav.png}};

\node[mt, label=Spectral features] (Spect) at (4,0)
    {\includegraphics[width=.2\textwidth]{imgs/spect.png}};
\draw [->, ArrowC2] (Audio) -- (Spect);


\node[ct] (DNN1) at (7,1.3) {$DNN_1$};
\node[ct, below=0.1cm of DNN1] (DNN2) {$DNN_2$};
\node[below=0.1cm of DNN2] (DNN3) {$\dots$};
\node[ct, below=0.1cmof DNN3] (DNNN) {$DNN_N$};
\node  [mt, fit={(DNN1) (DNN2) (DNNN) (DNNN)}, label=E2E ensemble] (E2E)  {};

\draw [->, ArrowC2] (Spect) -- (E2E);

\node[mt, label=Saliency maps] (Saliency) at (10.,0)
    {\includegraphics[width=.2\textwidth]{imgs/model_5_train_avg_grad_cb}};
    
\draw [->, ArrowC2] (E2E) -- (Saliency);

\node[mt, label=Feature selection] (FS) at (4,-4)
    {\includegraphics[width=.2\textwidth]{imgs/spect.png}};
%draw some markings on the spect
\draw[draw=red] (2.7,-4) -- (2.7,-4.1) -- (5.3,-4.1) -- (5.3,-4) -- (2.7,-4);

\draw[draw=red] (2.7,-4.7) -- (2.7,-4.8) -- (5.3,-4.8) -- (5.3,-4.7) -- (2.7,-4.7);



\draw [->, ArrowC2] (Spect) -- (FS);
\draw [->, ArrowC2] (Saliency) -- (10,-2.5) -- (5,-2.5) -- (FS);


\node[ct] (SDNN1) at (7,-3.5) {$DNN_1$};
\node[ct, below=0.1cm of SDNN1] (SDNN2) {$DNN_2$};
\node[below=0.1cm of SDNN2] (SDNN3) {$\dots$};
\node[ct, below=0.1cm of SDNN3] (SDNNN) {$DNN_N$};
\node  [mt, fit={(SDNN1) (SDNN2) (SDNN3) (SDNNN)}, label=E2E ensemble] (SE2E)  {};

\draw [->, ArrowC2] (5.3,-4.05) -- (SE2E);
\draw [->, ArrowC2] (5.3,-4.75) -- (SE2E);

\end{tikzpicture}
